Deep Multimodal Fusion by Channel Exchanging

Deep multimodal fusion by using multiple sources of data for classification or regression has exhibited a clear advantage over the unimodal counterpart on various applications. Yet, current methods including aggregation-based and alignment-based fusion are still inadequate in balancing the trade-off between inter-modal fusion and intra-modal processing, incurring a bottleneck of performance improvement. To this end, this paper proposes Channel-Exchanging-Network (CEN), a parameter-free multimodal fusion framework that dynamically exchanges channels between sub-networks of different modalities. Specifically, the channel exchanging process is self-guided by individual channel importance that is measured by the magnitude of Batch-Normalization (BN) scaling factor during training. The validity of such exchanging process is also guaranteed by sharing convolutional filters yet keeping separate BN layers across modalities, which, as an add-on benefit, allows our multimodal architecture to be almost as compact as a unimodal network. Extensive experiments on semantic segmentation via RGB-D data and image translation through multi-domain input verify the effectiveness of our CEN compared to current state-of-the-art methods. Detailed ablation studies have also been carried out, which provably affirm the advantage of each component we propose. Our code is available at https://github.com/yikaiw/CEN.

==> tabs/task_baselines.tex <==
\begin{table}[h]
\centering

\caption{}
\vspace{-0.3em}
\resizebox{103mm}{!}{
\begin{tabular}{p{1.7cm}p{2cm}p{2.5cm}|p{1cm}p{2cm}p{1cm}}%p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}}%{p{1.9cm}p{1.5cm}|p{1.3cm}p{1cm}|p{1.7cm}p{1.5cm}p{1.5cm}} 

\toprule
%\multirow{2}*{Modality}&\multirow{2}*{Approach}&\multicolumn{4}{c|}{Individual Training}&\multicolumn{4}{c}{Parallel Training}\\
%\multirow{2}{*}{Modality}&\multirow{2}{*}{Approach}& \multicolumn{8}{c|}{Fusion on an Encoder Layer} & \multicolumn{8}{c}{Fusion on a Decoder Layer}\\
%&&1&2&3&4&5&6&7&8&1&2&3&4&5&6&7&8\\
Task&Modality&Approach&L1 loss&L2 loss\\%&enc3&enc4&enc5&enc6&enc7&enc8\\
\midrule
\midrule
\multirow{5}{*}{Normals}&\multirow{5}{*}{\makecell[l]{RGB+Shade\\$\;$$\;$$\to$Normal}} 
& Concat (early)&0.133&0.086\\
&& Concat (middle)&0.122&0.070\\
&& Concat (late)&0.139&0.083\\
%&& Concat (multi-layer)\\
&& Concat (all-layer)&0.126&0.079\\
\cmidrule(r){3-5}
&& Ours&0.112&0.058\\
\midrule
\multirow{5}{*}{Reshading}&\multirow{5}{*}{\makecell[l]{RGB+Normal\\$\;$$\;$$\to$Shade}} 
& Concat (early)&0.156&0.060\\
&& Concat (middle)&0.138&0.045\\
&& Concat (late)&0.130&0.033\\
%&& Concat (multi-layer)\\
&& Concat (all-layer)&0.125&0.031\\
\cmidrule(r){3-5}
&& Ours&0.107&0.022\\
%& Ours&\multicolumn{16}{c}{1.17}\\
\midrule
\multirow{4}{*}{In-painting}&\multirow{2}{*}{\makecell[l]{Shade+Normal\\$\;$$\;$$\to$RGB}} 
& Concat&\\
&& Ours&\\
%& Ours&\multicolumn{16}{c}{}\\
\cmidrule(r){2-5}
&\multirow{2}{*}{\makecell[l]{Shade+Texture\\$\;$$\;$$\to$RGB}} 
& Concat&\\
&& Ours&\\
%& Ours&\multicolumn{16}{c}{}\\

\bottomrule
\end{tabular}}
\vspace{-1em}
\label{tabs:seg_results}

\end{table}

